Simulated Annealing for Optimal Resource Allocation in Wireless Networks with ImperfectCommunications

Simulated annealing (SA) method has had significant recent success in designing distributed control algorithms for wireless networks. These SA based techniques formed the basis of new CSMA algorithms and gave rise to the development of numerous variants to achieve the best system performance accommodating different communication technologies and more realistic system conditions. However, these algorithms do not readily extend to networks with noisy environments, as unreliable communication prevents them from gathering the necessary system state information needed to execute the algorithm. In recognition of this challenge, we propose a new SA algorithm that is designed to work more robustly in networks with communications that experience frequent message drops. The main idea of the proposed algorithm is a novel coupling technique that takes into account the external randomness of message passing failure events as a part of probabilistic uncertainty inherent in stochastic acceptance criterion of SA. As a result, the algorithm can be executed even with partial observation of system states, which was not possible under the traditional SA approach. We show that the newly proposed algorithm finds the optimal solution almost surely under the standard annealing framework while offering significant performance benefits in terms of its computational speed in the presence of frequent message drops.

==> proof.tex <==
\subsection{Optimality and efficiency}

Although the improvement of convergence speed due to the new algorithm is well expected, it is not clear whether the algorithm is desirable to find the optimal solution. Unfortunately, the algorithm does not necessarily achieve the same stationary probability distribution $\pi$ we intended, and it is difficult to find a closed form solution for it.
Technically speaking, the new algorithm experiences \emph{bias} to the desired stationary distribution due to the additional transitions we added onto the algorithm. Our main concern here is therefore to see if the algorithm is able to achieve the optimality under the conventional simulated annealing framework. To that end, we adopt a technical method introduced in \cite{connors1989simulated}, in which the optimality of the original simulated annealing algorithm is proved. We begin with introducing some necessary conditions and important results therein, and extend them to show the same optimality result for our case. 

The authors in \cite{connors1989simulated} have considered the following class of Markov chains of which transition probabilities can be written as
\begin{equation}
    p_{ij}(t) = c_{ij} \epsilon(t)^{V_{ij}}, \label{eq:trans_pr}
\end{equation}
where $V_{ij}, c_{ij} \geq 0,$ for all $i,j$, $\sum_{j \neq i} c_{ij} = 1$, for all $i$, $p_{ii}(t) = 1 - \sum_{j \neq i} p_{ij}(t)$, and $0 \leq \epsilon(t) \leq 1$, $t \geq 1$ is the parameter related to the cooling schedule. 
Note that the conventional simulated annealing algorithm can be represented by this form with setting $V_{ij} = [f(j) - f(i)]^+$ in which minimum $f(\cdot)$ is sought.
Here we focus on the popularly used inverse logarithmic cooling schedule, i.e., $\epsilon(t) = t^{-d}$, where $d > 0$ is some constant.
For this class of Markov chain, the authors have introduced the notion of \emph{recurrence orders} for the states and transitions of the Markov chain, as follows,

%We assume that the inverse logarithmic schedule is used, i.e., $\epsilon(t) = t^{-1/\rho}$, $t \geq 1$ where $\rho$ is the depth of the problem defined as follow: $\rho$ is the least number such that for any $i \in \Omega$, there exists a path $i_0 = i,i_1,\ldots,i_p = i^* \in \Omega^*$

\begin{definition}
The order of recurrence of a state $i \in \Omega$, denoted $\alpha_i$, is
\small
\begin{eqnarray*}
\alpha_i := \begin{cases} -\infty, &\mbox{if}~\sum_{t=0}^{\infty} \pi_i(t) < \infty, \\
  p^{-}, &\mbox{if}~p=\sup\left\{ c \geq 0 : \sum_{t=0}^{\infty} \epsilon(t)^c \pi_i(t) = \infty \right\}\\
  & ~\mbox{and}~\sum_{t=0}^{\infty}\epsilon(t)^p \pi_i(t) < \infty, \\
  p &\mbox{if}~p=\max\left\{ c \geq 0 : \sum_{t=0}^{\infty} \epsilon(t)^c \pi_i(t)= \infty \right\}
\end{cases} 
\end{eqnarray*}
\normalsize
\end{definition}
where $\pi_i(t) = \pr\{X(t) = i\}$ and $p$ is regarded as strictly larger than $p^-$, i.e., $p > p^- > p - \delta_0$ for some $\delta_0 > 0$.
Similarly, the \emph{order of recurrence of the transition from $i$ to $j$} is defined by,

\begin{definition}
The order of recurrence of the transition from $i$ to $j$, denoted $\alpha_{ij}$, is
\small
\begin{eqnarray*}
\alpha_{ij} := \begin{cases} -\infty, &\mbox{if}~\sum_{t=0}^{\infty} \pi_{ij}(t) < \infty, \\
  p^{-}, &\mbox{if}~p=\sup\left\{ c \geq 0 : \sum_{t=0}^{\infty} \epsilon(t)^c \pi_{ij}(t) = \infty \right\}\\
  & ~\mbox{and}~\sum_{t=0}^{\infty}\epsilon(t)^p \pi_{ij}(t) <  \infty, \\
  p &\mbox{if}~p=\max\left\{ c \geq 0 : \sum_{t=0}^{\infty} \epsilon(t)^c \pi_{ij}(t)= \infty \right\}
\end{cases} 
\end{eqnarray*}
\normalsize
\end{definition}
where $\pi_{ij}(t) = \pr\{X(t)=i, X(t+1)=j\}$.
They also defined $\rho$, the \emph{order of cooling} of $\{\epsilon(t)\}$, as follows.
\begin{definition}
The order of the cooling schedule $\{\epsilon(t)\}$, denoted $\rho$, is defined as
\small
\begin{eqnarray*}
\rho := \begin{cases} -\infty, &\mbox{if}~\sum_{t=0}^{\infty} \epsilon(t) < \infty, \\
  p^{-}, &\mbox{if}~p=\sup\left\{ c \geq 0 : \sum_{t=0}^{\infty} \epsilon(t)^c  = \infty \right\} \\
  & ~\mbox{and}~\sum_{t=0}^{\infty}\epsilon(t)^p  < \infty, \\
  p &\mbox{if}~p=\max\left\{ c \geq 0 : \sum_{t=0}^{\infty} \epsilon(t)^c = \infty \right\}
\end{cases} 
\end{eqnarray*}
\normalsize
\end{definition}

Having defined the above terms, we summarize important results established in \cite{connors1989simulated} as well as in \cite{connors1988balance}, which are valid under the following mild assumptions.

\textbf{Assumptions}
\begin{enumerate}
    \item $d \geq ...$
    \item $\exists \; j \in N_i \; \Leftrightarrow \; \exists \; i \in N_j \; \forall i,j \in \Omega$
\end{enumerate}

\begin{lemma} \cite{connors1989simulated, connors1988balance} Under the above assumptions, it holds
\begin{enumerate} %[label=(\roman*)]
\item Relation between $\alpha_i$ and $\alpha_{ij}$.
    \begin{align} \label{eq:prev_results1}
        \alpha_{ij} = \alpha_i \ominus V_{ij} ~~\mbox{for all}~i,j \in \Omega,
    \end{align}
    where the operation "$\ominus$" is defined such that $a \ominus b := a-b$ if $a \geq b$, and $a \ominus b := - \infty$ if $a < b$.
\item $d = \max_{i \in \Omega} \; \alpha_i = \rho$, where $\alpha_i = \rho$ if and only if $i \in \Omega^*$.
\item Let $S$ be the set of states in the largest orders of recurrence, i.e., $S := \{ i \in \Omega : \alpha_i = \rho\}$. Then,
    \begin{align}
        \lim_{T \rightarrow \infty} \frac{1}{T} \sum_{t=1}^T \pr\{X(t) \in S\} = 1. \label{eq:prev_results3}
    \end{align}
\end{enumerate}
\end{lemma}

Note that the transition probability of the basic algorithm in Algorithm \ref{alg:basic}, $P(\x,\x')$, can be represented by the form in eq. (\ref{eq:trans_pr}) by setting $\Omega := \bX$, $i:= \x$, $j:=\x'$, $p_{ij} := P(\x,\x')$, $c_{ij} := c(\x,\x')$, $V_{ij} := V(\x,\x') = [f(\x')-f(\x)]^+$, and with re-parameterization $\epsilon(t) = e^{-\beta(t)}$, which also reconfirms the validity of Colollary \ref{cor:basic}. However, eq. (\ref{eq:trans_pr}) cannot represent the dynamics of RSA algorithm as described in eq. (\ref{eq:trans_pr_rsa}).
To pursue the above approach to analyzing the optimality of RSA algorithm, it is necessary to consider a more general class of Markov chain which has transition probabilities of the form,
\begin{align} 
    p_{ij}(t) = c_{ij} \sum_{m \in M^{ij}} a_{ij}(m) \epsilon(t)^{V^{m}_{ij}}, 
\end{align}
where $M^{ij}$ is some finite set associated with the transition from $i$ to $j$, $i,j \in \Omega$, $V^{m}_{ij} \geq 0$ for all $m \in M^{ij}$, and $a_{ij}(m) \in (0,1]$ is some probability of an element $m \in M^{ij}$ defined over its sample space $M^{ij}$.
This form covers that of $P^R(\x,\x')$ by setting $M^{ij} := \mathcal{P}(N_{i'})$, $m := S \in \mathcal{P}(N_{i'})$, $a_{ij}(m) := q_{i', [S]}$, for $i = \x$ and $j = \x'$, $V^m_{ij} := V^S(\x,\x')$, where $\mathcal{P}(A)$ is the powerset of set $A$, and $i'$ corresponds to $i$ in eq. (\ref{eq:trans_pr_rsa}).
For this form, we obtain the generalized correspondence of eq. (\ref{eq:prev_results1}) where we provide its proof is in the Appendix.

\begin{lemma} \label{lem:general}
$\alpha_{ij} = \alpha_{i} \ominus \inf_{m \in M^{ij}} V^m_{ij}, \;\; \forall i,j \in \Omega.$
\end{lemma}


Let $\alpha(\x)$ and $\alpha(\x,\x')$ be the recurrence rate order of state $\x$ and that of state transition from $\x$ to $\x'$, for any $\x,\x' \in \Omega$ due to the Markov chain induced by the Basic Algorithm in Algorithm \ref{alg:basic}, and let $\hat{\alpha}(\x)$ and $\hat{\alpha}(\x,\x')$ be those from RSA algorithm, respectively. In the following lemma, we verify that all the recurrence orders for any state and transition are equivalent between the two algorithms.

\begin{lemma} \label{lem:equiv}
$\alpha(\x) = \hat{\alpha}(\x), \; \text{and} \; \alpha(\x,\x') = \hat{\alpha}(\x,\x')$, for all $\x,\x' \in \Omega$, 
\end{lemma}

We establish the following theorem of which proof immediately follows due to Lemma \ref{lem:general}, \ref{lem:equiv} and the results in eq (\ref{eq:prev_results2}-\ref{eq:prev_results4}).

\begin{theorem}
RSA algorithm is annealing optimal.
\end{theorem}

Furthermore, since the transition probability of LSA algorithm can be represented as a special instance of that of RSA algorithm, one can easily see that LSA algorithm not necessarily with symmetric proposal distribution is also annealing optimal.

\begin{corollary}
LSA algorithm is annealing optimal.
\end{corollary}

Regarding the efficiency in terms of convergence speed, we look at the following quantity to compare different algorithms,
\begin{eqnarray*}
H(\x,\x') \triangleq \inf \{ k \in \mathbb{N} : X_t = \x, X_{t+k} = \x'\},
\end{eqnarray*}
which is the number of transitions needed from a state $\x$ until to hit any other state $\x'$. 
Let $H^{L}$, $H^{R}$, $H^{B}$ be the above defined hitting times that can be obtained from LSA, RSA, and the basic algorithm, resepectively.
Due to simple coupling argument, one can easily obtain the following.
\begin{theorem} For any $\x,\x' \in \bX$, it holds
    \begin{equation*}
        H^{L}(\x,\x') \geq H^{R}(\x,\x') \geq H^{B}(\x,\x').
    \end{equation*}
\end{theorem}
